Robust Empirical Risk Minimization with Tolerance

Developing simple, sample-efficient learning algorithms for robust classification is a pressing issue in today's tech-dominated world, and current theoretical techniques requiring exponential sample complexity and complicated improper learning rules fall far from answering the need. In this work we study the fundamental paradigm of (robust) $\textit{empirical risk minimization}$ (RERM), a simple process in which the learner outputs any hypothesis minimizing its training error. RERM famously fails to robustly learn VC classes (Montasser et al., 2019a), a bound we show extends even to `nice' settings such as (bounded) halfspaces. As such, we study a recent relaxation of the robust model called $\textit{tolerant}$ robust learning (Ashtiani et al., 2022) where the output classifier is compared to the best achievable error over slightly larger perturbation sets. We show that under geometric niceness conditions, a natural tolerant variant of RERM is indeed sufficient for $\gamma$-tolerant robust learning VC classes over $\mathbb{R}^d$, and requires only $\tilde{O}\left( \frac{VC(H)d\log \frac{D}{\gamma\delta}}{\epsilon^2}\right)$ samples for robustness regions of (maximum) diameter $D$.

==> 1_intro.tex <==
%!TEX root = main.tex
\section{Introduction}

Adversarially robust classification has become a staple of modern machine learning. Here, the goal is to learn a classifier that is not only accurate but also robust to perturbations of the input. Finding algorithms in this setting with provable guarantees has recently been an important research direction both for parametric \citep{loh18, attias19, Srebro19, bartlett19, pathak20} and non-parametric \citep{WJC18, YRWC19, Bhattacharjee20, Bhattacharjee21} classifiers. 

In the parametric case, \citet{Omar19} showed that there exist finite VC classes, $\mathcal{H}$, where no proper learning algorithm can converge towards the optimal classifier, even with arbitrary amounts of training data. To circumvent this, they provide an alternative \textit{improper} learning algorithm based on sample compression and boosting that is able to provide PAC-like guarantees for robustness. Furthermore, their algorithm works for arbitrary choices of \textit{robustness regions} -- for a data point $x$, its robustness region, $U_x$, is the set of points that must be classified identically to $x$ in order to be robust at $x$.

While certainly a breakthrough in its own right, \citet{Omar19}’s work nevertheless has several drawbacks; their algorithm's sample complexity is potentially exponential in the VC dimension of $\mathcal{H}$, and utilizes a complicated improper learning rule. 

To mitigate these issues, \citet{Urner22} introduced the notion of robust classification with \textit{tolerance}. In the specific case where the robustness region of each $x$, $U_x$, is a ball of radius $r$ centered at $x$, they propose that the error of the learner be compared to the best achievable error for balls of radius $r(1 + \gamma)$ where $\gamma > 0$ is the tolerance parameter. Under this framework, they are able to give an algorithm with PAC-guarantees with a significantly improved sample complexity. Furthermore, they are able to limit their interaction with the robustness regions, $U_x$, to a \textit{sampling oracle}, which draws points from $U_x$ at uniform according to some fixed measure. 

However, their algorithm is still an improper learning rule that leverages the sample compression techniques used in \citet{Omar19}. Additionally, by only considering the case where $u_x$ is a ball of radius $r$, they give up a substantial amount of generality that \citet{Omar19}'s algorithm included. 

This motivates our work, where we seek to generalize the notion of robust learning with tolerance to \textit{arbitrary} robustness regions, and to find conditions under which simpler, \textit{proper} learning methods suffice. 

We begin by introducing the notion of \textit{perturbed robustness regions}, $U_x^\gamma$, where $\gamma > 0$ is a distance in the $\ell_2$ metric. The perturbed region can be defined as all points that have distance at most $\gamma$ from some point in the original robustness region, $U_x$. $U_x^\gamma$ can be thought of as a natural generalization to the balls of increased radii considered in \citet{Urner22}. Our goal then becomes to learn a classifier that has error competitive with the best achievable error with respect to the perturbed regions, $U_x^\gamma$. 

Next, we show that under certain regularity conditions on our hypothesis class, $\cH$, robust learning with tolerance is possible with a surprisingly simple algorithm that we call $TolRERM$. We first sample $r \sim [0, \gamma]$ at random, and then perform \textit{robust empirical risk minimization} using the perturbed robustness regions, $U_x^r$. 

This algorithm achieves a sample complexity of $O\left(\frac{vd\log \frac{dD}{\epsilon\gamma\delta}}{\epsilon^2}\right)$ for robust classification over $\R^d$, where $v$ denotes the VC-dimension of $\cH$ and $D$ denotes the maximum diameter of any robustness region $U_x$. Our algorithm matches the sample complexity given in \citet{Urner22} up to logarithmic factors but enjoys the additional benefits of applying to general robustness regions along with being a proper learning algorithm (as we output a classifier $h \in \cH$). 

Our algorithm does require a single use of a robust empirical risk minimization oracle with respect to $U^r$, the randomly perturbed robustness regions. While this oracle poses a potentially stronger mode of interaction with the robustness regions than the sampling oracle used in \citet{Urner22}, we show that such a strengthening is inevitable. Due to the unknown nature of our robustness regions, $U_x$, we show that there exists hypothesis classes where $\Omega((\frac{D}{\gamma})^d)$ queries to a sampling oracle are required for robust learning with tolerance if no other interaction with $U_x$ is permitted. 



==> Intro2.tex <==
%!TEX root = main.tex
\section{Introduction}

Adversarially robust classification is a staple of modern machine learning. In the robust setting, along with meeting standard accuracy guarantees over a given hypothesis class $\mathcal{H}$ (binary labelings over a ground set $X$), predictions made by a learner at test time must additionally be robust to adversarial perturbations to the input, typically defined by a fixed family $\mathcal{U}=\{U_x\}_{x \in X}$ of possible perturbations. Developing robust algorithms with provable guarantees has been an important research direction in recent years, both for parametric \cite{loh18, attias19, Srebro19, bartlett19, pathak20} and non-parametric \cite{WJC18, YRWC19, Bhattacharjee20, Bhattacharjee21} classifiers, but understanding the performance of even the most basic algorithms in the setting remains widely open.

In this work, we study one of the simplest, most fundamental algorithmic paradigms in learning, a classical method called \textit{empirical risk minimization} (ERM). In the robust setting, algorithm is said to be an empirical risk minimizer (RERM) if it always outputs a hypothesis in the class with minimal \textit{robust} risk over its training data. In the standard setting, it is a classical result that any learnable class is learnable (near-optimally) by any ERM. Unfortunately, this is known to fail drastically in the robust setting---\citet{Omar19} showed that there exist finite VC classes, $\mathcal{H}$, where no algorithm outputting hypotheses in $\mathcal{H}$ (called a \textit{proper} learner) can converge towards the optimal classifier, even with arbitrary amounts of training data. Conversely, such classes \textit{are} in fact robustly learnable, but require complicated improper learning rules and a potentially exponential number of samples.

The failure of Robust ERM for general classes raises an interesting question: \textit{are there natural sufficient conditions for the success of RERM?} One might hope, for instance, that the method works over any sufficiently `nice' hypothesis class. In this sense \citet{Omar19}’s lower bound is no barrier, as it shows the failure of RERM only for a fairly pathological example. Sadly, this is not the case. We show that RERM (indeed any proper algorithm) fails even for settings as simple as (bounded) linear classifiers.
\begin{thm}[Failure of RERM for Linear Classifiers]\label{thm:intro1}
For any $W>0$ and $d>1$, let $\cH_W$ denote the set of linear classifiers with distance at most $W$ from the origin. Then there exists a set of robustness regions $U$ over $\R^d$ such that for any proper learning algorithm $L$ there exists a distribution $\cD$ for which the following hold:
\begin{itemize}
	\item \textbf{$\cD$ is realizable}: There exists $h^* \in \cH_W$ such that $\ell_U(h^*, \cD) = 0$.
	\item \textbf{$L$ has high error}: With probability at least $\frac{1}{7}$ over $S \sim \cD^m$, $\ell_U(L(S), \cD) > \frac{1}{8}$. 
\end{itemize}
\end{thm}

With this in mind, another promising approach is to instead relax the notion of robustness. We'll consider a recent model of \citet{Urner22} called \textit{tolerant} robust learning. In the tolerant setting, the learner is only required to compete with the best loss over a relaxed family of perturbation sets $\mathcal{U}^\gamma$ for a (potentially arbitrary) tolerance parameter $\gamma >0$. \citet{Urner22} studied this setting in the special case of radius $r$ balls, where the learner competes with robust error against $r(1 + \gamma)$-balls. Under this framework, \citet{Urner22} give an algorithm with PAC-guarantees for VC classes using significantly fewer samples, but the techniques remain improper and only hold for the simplest robustness setting.

In this work, we show that a simple variant of RERM in the tolerant model succeeds under natural conditions on the hypothesis class. In particular, we study a notion of smoothness called \textit{regularity}, which roughly promises that every point in the instance space should be contained in some ball of the same label. This captures many well-studied settings such as compact, differential manifolds in $\mathbb{R}^d$.
\begin{thm}[Tolerant RERM for Regular Classes]\label{thm:upper_bound}
Let $\cH$ be a regular hypothesis class with VC dimension $v$ over $\mathbb{R}^d$, and let $\mathcal{U}$ be any set of robustness regions. Then $TolRERM$ tolerantly PAC-learns $(\cH, \mathcal{U})$ with tolerant sample complexity 
\[
m(\epsilon, \delta, \gamma)  = O\left( \frac{vd\log \frac{d\text{Diam}(U)}{\epsilon\gamma\delta}}{\epsilon^2}\right),
\]
where $\text{Diam}(U)$ denotes the maximum $\ell_2$ diameter across robustness regions $U_x$. 
\end{thm}
Theorem \ref{thm:upper_bound} matches the sample complexity given in \citet{Urner22} up to logarithmic factors and enjoys the additional benefits of applying to more general robustness regions along with its algorithmic simplicity (not to mention properness). Finally it's worth noting that while \citet{Urner22} only requires sampling access to the perturbation sets, stronger access such as an empirical risk minimizer is inevitable in the general setting where $\mathcal{U}$ is unknown. We show that there exists hypothesis classes where $\Omega((\frac{D}{\gamma})^d)$ queries to a sampling oracle are required for robust learning with tolerance if no other interaction with $U_x$ is permitted.  

While Theorem \ref{thm:upper_bound} gives a natural sufficient condition for the success of RERM in relaxed settings, many questions in this direction remain wide open. It would be interesting to identify a condition under which success of RERM is also necessary, both in the tolerant and original robust models. Furthermore, it should be noted that while we prove RERM fails to learn nice classes in the latter, the perturbation family we use to achieve this is highly combinatorial. As such, there is still hope that RERM may be sufficient in the traditional setting under \textit{joint} niceness conditions on $\mathcal{H}$ and $\mathcal{U}$, though the close interplay between the two families seems to make identifying such a condition difficult, if it is indeed possible.
